Kinetics of interactions of matter, antimatter and radiation consistent with antisymmetric (CPT-invariant) thermodynamics

This work investigates the influence of directional properties of decoherence on kinetics rate equations. The physical reality is understood as a chain of unitary and decoherence events. The former are quantum-deterministic, while the latter introduce uncertainty and increase entropy. For interactions of matter and antimatter, two approaches are considered: symmetric decoherence, which corresponds to conventional symmetric (CP-invariant) thermodynamics, and antisymmetric decoherence, which corresponds to antisymmetric (CPT-invariant) thermodynamics. Radiation, in its interactions with matter and antimatter, is shown to be decoherence-neutral. The symmetric and antisymmetric assumptions result in different interactions of radiation with matter and antimatter. The theoretical predictions for these differences are testable by comparing absorption (emission) of light by thermodynamic systems made of matter and antimatter. Canonical typicality for quantum mixtures is briefly discussed in the Appendix.

==> fig8.tex <==

\begin{figure}[h]
\begin{center}
\includegraphics[width=10cm,page=7,trim=0cm 3.8cm 0cm 8.6cm, clip ]{figs}
\caption{Two-state interpretatuon of quantum mechanical events: complete measurements and decoherence are connected by unitary evolutions.}
\label{fig8}
\end{center}
\end{figure}


%\includegraphics[width=8.5cm,page=1,trim=3.1cm 4.3cm 2cm 5.3cm, clip ]{figs}

